Offline Retrieval Evaluation Without Evaluation Metrics

Offline evaluation of information retrieval and recommendation has traditionally focused on distilling the quality of a ranking into a scalar metric such as average precision or normalized discounted cumulative gain. We can use this metric to compare the performance of multiple systems for the same request. Although evaluation metrics provide a convenient summary of system performance, they also collapse subtle differences across users into a single number and can carry assumptions about user behavior and utility not supported across retrieval scenarios. We propose recall-paired preference (RPP), a metric-free evaluation method based on directly computing a preference between ranked lists. RPP simulates multiple user subpopulations per query and compares systems across these pseudo-populations. Our results across multiple search and recommendation tasks demonstrate that RPP substantially improves discriminative power while correlating well with existing metrics and being equally robust to incomplete data.

==> rpp-section/comparison.tex <==
\subsection{Comparison to Existing Metrics}
In this section, we compare RPP to the methods presented in Section \ref{sec:preliminaries}.
% RPP uses only the rank position of relevant items to infer preferences, without modeling user fatigue with a technique like position-discounting.  Moreover, grade information is used to model different populations, not item preferences.  %As such, we are interested in comparing RPP to  existing retrieval metrics.  

To begin, we can compare RPP with metric-based evaluation by analyzing how the disaggregated metric $\dmetric_i$ (Section \ref{sec:motivation}) changes as a function of $i$.  Figure \ref{tab:disaggregated-metrics} contains the disaggregated values for several standard evaluation metrics.  These expressions encode the relative weight allocated to different pseudo-populations $\users_i$.  Standard evaluation metrics such as RBP, AP, DCG, and RR all observe the largest contribution to metric differences at the highest rank positions.  Even AP, which modulates the difference in inverse positions with a multiplicative recall level factor $i$ is dominated by diminishing differences at low ranks.  This confirms our claim of poor label efficiency (since relevant items at lower rank positions can contribute less)
and poor robustness to user behavior (since the performance difference for users interested in higher recall levels is negligible).  RR, ISL, and TSL also exhibit poor label efficiency and robustness to user behavior since, by design, they exclude all but a single difference.  Meanwhile, ASL will tend to have the opposite effect of emphasizing differences at lower ranks since, at these higher recall levels, $\rpx_i$ and $\rpy_i$ are likely to be separated by many more rank positions than earlier recall levels.   In contrast, for RPP, the disaggregated magnitude is fixed across recall levels, resulting in both label efficiency (since all relevant items contribute equally regardless of rank position) and robustness to user behavior (since the performance differences for users at all recall levels contribute equally).

To illustrate the implication of these position biases, we can see how $\dmetric_i$ changes for two hypothetical rankings, $a$ and $b$.  In the left-hand plot of Figure \ref{fig:delta-metrics}, we depict the uninterpolated precision-recall curves for $a$ and $b$.    Whereas AP approximates the area under the  uninterpolated precision-recall curve, RPP can be interpreted as a sign test at sampled recall levels, similar to approaches taken for ROC curves \cite{braun:roc-sign}.


In the right-hand plot of Figure \ref{fig:delta-metrics}, we present $\dmetric_i(a,b)$ as a function of $i$.  Notice that almost every traditional metric, including `recall-oriented' metrics like AP, allocate most of the mass to the top position.  Conversely, ASL allocates more weight to later values of $i$.  RPP, on the other hand, treats all recall levels equally.  



\begin{figure}
    \centering
    {
        \renewcommand{\arraystretch}{1.5}

    \begin{subtable}[b]{\linewidth}
        \centering
        \caption{Disaggregated recall-paired metrics}\label{tab:disaggregated-metrics}
        {\footnotesize
        \begin{tabular}{lc}
            metric & $\dmetric_i$\\
            \hline
            RBP \cite{moffat:rbp} & $\gamma^{\rpx_i} - \gamma^{\rpy_i}$\\
            AP & $i\left(\frac{1}{\rpx_i} - \frac{1}{\rpy_i}\right)$\\
            NDCG  \cite{NDCG}& $\frac{1}{\log_2(\rpx_i+1)} - \frac{1}{\log_2(\rpy_i+1)}$\\
            RR  & $\frac{1}{\rpx_i} - \frac{1}{\rpy_i}, (i=1)$ \\
            ISL \cite{cooper:esl} & $\rpy_i - \rpx_i, (i=1)$\\
            TSL \cite{cooper:esl} & $\rpy_i - \rpx_i, (i=\nrel)$\\
            ASL, bpref \cite{rocchio:thesis,buckley:evaluation-with-incomplete-information,alex:asl}& $\rpy_i - \rpx_i$\\
            RPP & $\text{sgn}(\rpy_i - \rpx_i)$\\
            \hline
        \end{tabular}
        }
    \end{subtable}
    }

    \begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[width=3.25in]{rpp-section/graphics/delta-metrics.pdf}
        \caption{Metric differences for two systems' rankings of one request with six relevant items. }\label{fig:delta-metrics}
    \end{subfigure}
    \caption{Disaggregated metric behavior.}
\end{figure}

Although position-based metrics like ASL more evenly allocate weight across recall levels, \citet{magdy:pres} note that the range of this metric can be quite large, sensitive to outliers, and difficult to reason with.  Unretrieved items, often assumed to be ranked at the bottom of a ranking of the full corpus (Section \ref{sec:preliminaries}), can exacerbate the variance in the metric, even for moderately sized corpora.  In contrast, RPP, because it only considers relative positions, can be computed without an exact corpus size.

In comparison to interleaving, while Equations \ref{eq:interleaving} and \ref{eq:rpp} appear  similar, there are a few important differences.  First, the event space for interleaving is the set of all rank positions rather than the set of all recall levels.  This subtle difference means that interleaving emphasizes the number of relevant items collected at a rank position rather than the effort taken to collect the same number of relevant items.  Moreover, in online interleaving, because $p(k)$ is derived from behavioral data, it will be skewed toward higher rank positions (i.e. users introduce position bias) and preferences at lower positions will be overshadowed by those in higher positions.
% , resulting in lower robustness to user behavior.
% By controlling $p(k)$ in OI, 

% .  We will revisit this in the context of offline interleaving in Section \ref{sec:results:metric-correlation}.  
% The difference in $\ap$ between $\rlx$ and $\rly$ can be defined by,
% \begin{align}
%     \pap(\rlx,\rly) &= \sum_{i=1}^{\nrel} p(\users_i)i\left(\frac{1}{\esl_i(\rlx)}-\frac{1}{\esl_i(\rly)}\right)
% \end{align}
% Notice that we are aggregating a preference for each user pseudo-population $i$.  However, even though each population weights grow linearly in $i$, this is dominated by the  degradation $\frac{1}{\esl_i(\rlx)}$, resulting in a minimal contribution from the users seeking more relevant items.  






